Drantal-NeRF: Diffusion-Based Restoration for Anti-aliasing Neural Radiance Field

Aliasing artifacts in renderings produced by Neural Radiance Field (NeRF) is a long-standing but complex issue in the field of 3D implicit representation, which arises from a multitude of intricate causes and was mitigated by designing more advanced but complex scene parameterization methods before. In this paper, we present a Diffusion-based restoration method for anti-aliasing Neural Radiance Field (Drantal-NeRF). We consider the anti-aliasing issue from a low-level restoration perspective by viewing aliasing artifacts as a kind of degradation model added to clean ground truths. By leveraging the powerful prior knowledge encapsulated in diffusion model, we could restore the high-realism anti-aliasing renderings conditioned on aliased low-quality counterparts. We further employ a feature-wrapping operation to ensure multi-view restoration consistency and finetune the VAE decoder to better adapt to the scene-specific data distribution. Our proposed method is easy to implement and agnostic to various NeRF backbones. We conduct extensive experiments on challenging large-scale urban scenes as well as unbounded 360-degree scenes and achieve substantial qualitative and quantitative improvements.

==> Figures/first_page.tex <==
% CVPR 2024 Paper Template; see https://github.com/cvpr-org/author-kit
% \documentclass[runningheads]{llncs}

%%%%%%%%% PAPER TYPE  - PLEASE UPDATE FOR FINAL VERSION
% \usepackage{cvpr}              % To produce the CAMERA-READY version
% \usepackage[review]{eccv}      % To produce the REVIEW version
% \usepackage[pagenumbers]{cvpr} % To force page numbers, e.g. for an arXiv version

% Import additional packages in the preamble file, before hyperref
% \usepackage{multirow}
% \usepackage{nicefrac}
% \usepackage{graphicx}

% It is strongly recommended to use hyperref, especially for the review version.
% hyperref with option pagebackref eases the reviewers' job.
% Please disable hyperref *only* if you encounter grave issues, 
% e.g. with the file validation for the camera-ready version.
%
% If you comment hyperref and then uncomment it, you should delete *.aux before re-running LaTeX.
% (Or just hit 'q' on the first LaTeX run, let it finish, and you should be clear).
% \usepackage[pagebackref,breaklinks,colorlinks,citecolor=cvprblue]{hyperref}

%%%%%%%%% TITLE - PLEASE UPDATE
% \title{}

%%%%%%%%% AUTHORS - PLEASE UPDATE
% \author{First Author\\
% Institution1\\
% Institution1 address\\
% {\tt\small firstauthor@i1.org}
% For a paper whose authors are all at the same institution,
% omit the following lines up until the closing ``}''.
% Additional authors and addresses can be added with ``\and'',
% just like the second author.
% To save space, use either the email address or home page, not both
% \and
% Second Author\\
% Institution2\\
% First line of institution2 address\\
% {\tt\small secondauthor@i2.org}
% }

% \begin{document}

% \clearpage
\begin{figure*}[!ht]
	\small
	\centering
        \begin{minipage}[t]{0.23\linewidth}
		\centering
		\centerline{\includegraphics[width=0.99\linewidth]{Figures/vis_city/block_all_tensor_block_2_test_0007.png}}
		\vspace{-0.3mm}
		\centerline{TensoRF}
	\end{minipage}
	\begin{minipage}[t]{0.23\linewidth}
		\centering
		% \vspace{-44.6mm}
		\centerline{\includegraphics[width=0.99\linewidth]{Figures/vis_city/block_all_grid_block_2_test_0007.png}}
		\vspace{-0.3mm}
		\centerline{GridNeRF}
	\end{minipage}
	\begin{minipage}[t]{0.23\linewidth}
		\centering
		% \vspace{-44.6mm}
		\centerline{\includegraphics[width=0.99\linewidth]{Figures/vis_city/block_all_griddiff_block_2_test_0007.png}}
		\vspace{-0.3mm}
		\centerline{GridNeRF+\ours}
	\end{minipage}
	\begin{minipage}[t]{0.23\linewidth}
		\centering
		% \vspace{-44.6mm}
		\centerline{\includegraphics[width=0.99\linewidth]{Figures/vis_city/block_all_gt_block_2_test_0007.png}}
		\vspace{-0.3mm}
		\centerline{G.T.}
	\end{minipage}

     \vspace{+3mm}
 
 \begin{minipage}[t]{0.23\linewidth}
		\centering
		\centerline{\includegraphics[width=0.99\linewidth]{Figures/vis_360/color_cc_005_treehill_mipnerf360.png}}
		\vspace{-0.3mm}
		\centerline{MipNeRF-360}
	\end{minipage}
	\begin{minipage}[t]{0.23\linewidth}
		\centering
		% \vspace{-44.6mm}
		\centerline{\includegraphics[width=0.99\linewidth]{Figures/vis_360/color_cc_005_treehill_zipnerf.png}}
		\vspace{-0.3mm}
		\centerline{ZipNeRF}
	\end{minipage}
	\begin{minipage}[t]{0.23\linewidth}
		\centering
		% \vspace{-44.6mm}
		\centerline{\includegraphics[width=0.99\linewidth]{Figures/vis_360/color_cc_enhanced_005_treehill_zipnerfdiff.png}}
		\vspace{-0.3mm}
		\centerline{ZipNeRF+\ours}
	\end{minipage}
	\begin{minipage}[t]{0.23\linewidth}
		\centering
		% \vspace{-44.6mm}
		\centerline{\includegraphics[width=0.99\linewidth]{Figures/vis_360/color_005_treehill_gt.png}}
		\vspace{-0.3mm}
		\centerline{G.T.}
	\end{minipage}
 
	%\vspace{+2mm}
	\caption{Performance comparison of our proposed diffusion-based restoration for anti-aliasing Neural Radiance Field (\textbf{Drantal-NeRF}) with some state-of-the-art baselines~\cite{zipnerf, gridnerf, tensorf, miperf360}. Our proposed Drantal significantly helps mitigating the aliasing artifacts produced by other baselines. See the water surfaces, road lines and buildings in the top row, and the fences, leaves and backgrounds in the bottom row. Zoom in for better comparison.}
	\label{fig:firstpage}
	\vspace{-2mm}
\end{figure*}


% \end{document}

